Reachability Switching Games

We study the problem of deciding the winner of reachability switching games for zero-, one-, and two-player variants. Switching games provide a deterministic analogue of stochastic games. We show that the zero-player case is NL-hard, the one-player case is NP-complete, and that the two-player case is PSPACE-hard and in EXPTIME. For the zero-player case, we also show P-hardness for a succinctly-represented model that maintains the upper bound of NP $\cap$ coNP. For the one- and two-player cases, our results hold in both the natural, explicit model and succinctly-represented model. Our results show that the switching variant of a game is harder in complexity-theoretic terms than the corresponding stochastic version.

==> overview_figures/one.tex <==
% fill white since these will be used in the foreground
\tikzset{box/.style={draw, thick, minimum height=1.8cm,minimum width=0.5cm}}
\tikzstyle{component}=[fill=white, draw, thick, minimum size=0cm,align=center]
\tikzstyle{dest}=[fill=white, thick, minimum size=0cm,align=center]

\begin{tikzpicture}[
	decoration={markings,mark=at position 0.6 with {\arrow{triangle 60}}},
	path/.style={thick},
	clip=false
	%path/.style={ultra thick,>=stealth,postaction=decorate}
	%every node/.style={
]

% BOXES IN THE BACKGROUND
\begin{pgfonlayer}{background}
\node[box, xshift=0cm, yshift=0cm, align=center, text width=1.8cm] (contr) {Controller};
\end{pgfonlayer}{background}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% START
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\node[dest,xshift=-1cm] (start) at (contr.west) {start};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FAIL FROM CONTROLLER
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\node[dest,xshift=1cm,yshift=0cm] (fail) at (contr.east) {fail};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% VARIABLES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\node[component,xshift=-3cm,yshift=-1cm] (x1) at (contr.south) {$x_1$};
\node[component,xshift=-1cm,yshift=-1cm]  (x2) at (contr.south) {$x_2$};
\node[component,xshift=1cm,yshift=-1cm]  (x3) at (contr.south) {$x_3$};
\node[component,xshift=3cm,yshift=-1cm]  (x4) at (contr.south) {$x_4$};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TARGET
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\node[dest,xshift=1.5cm,yshift=0cm] (target) at (x4) {target};

%\node[xshift=-1cm,yshift=-0.75cm]  (bphantom) at (contr.south) {$\cdots$};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CLAUSES + extra starts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\node[component,xshift=0.5cm,yshift=-1cm]  (c1) at (x1.south) {$C_1$};
\node[component,xshift=1cm,yshift=-1cm]  (c2) at (x2.south) {$C_2$};
\node[component,xshift=3.5cm,yshift=-1cm]  (c3) at (x2.south) {$C_3$};

\node[dest,xshift=-1cm,yshift=-1cm]  (x1start) at (x1.south) {start};
\node[dest,xshift=0cm,yshift=-1cm]  (x3start) at (x3.south) {start};
\node[dest,xshift=0.5cm,yshift=-1cm]  (x4start) at (x4.south) {start};
\node[dest,xshift=1.5cm,yshift=-1cm]  (x4start2) at (x4.south) {start};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% START/FAIL FOR CLAUSES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\node[dest,xshift=-0.5cm,yshift=-1cm]  (c1start) at (c1.south) {start};
\node[dest,xshift=0.5cm,yshift=-1cm]  (c1fail) at (c1.south) {fail};

\node[dest,xshift=-0.5cm,yshift=-1cm]  (c2start) at (c2.south) {start};
\node[dest,xshift=0.5cm,yshift=-1cm]  (c2fail) at (c2.south) {fail};

\node[dest,xshift=-0.5cm,yshift=-1cm]  (c3start) at (c3.south) {start};
\node[dest,xshift=0.5cm,yshift=-1cm]  (c3fail) at (c3.south) {fail};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% EDGES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\draw[path,->] (start) -- (contr);
\draw[path,->] (contr) -- (fail);

% formula to x_i
\draw[path,->] (contr) -- node[right] {} (x1);
\draw[path,->] (contr) -- node[right] {} (x2);
\draw[path,->] (contr) -- node[right] {} (x3);
\draw[path,->] (contr) -- node[right] {} (x4);

% x_i to x_i+1
\draw[path,dashed,->] (x1) -- node[right] {} (x2);
\draw[path,dashed,->] (x2) -- node[right] {} (x3);
\draw[path,dashed,->] (x3) -- node[right] {} (x4);
\draw[path,dashed,->] (x4) -- node[right] {} (target);

\draw[path,->] (c1) -- node[right] {} (c1start);
\draw[path,->] (c1) -- node[right] {} (c1fail);
\draw[path,->] (c2) -- node[right] {} (c2start);
\draw[path,->] (c2) -- node[right] {} (c2fail);
\draw[path,->] (c3) -- node[right] {} (c3start);
\draw[path,->] (c3) -- node[right] {} (c3fail);

% edges from variables to clauses/start

% c1
\draw[path,->] (x1) -- node[right] {} (c1);
\draw[path,->] (x2) -- node[right] {} (c1);
%\draw[path,->] (x4) -- node[right] {} (c1);

% c2
\draw[path,->] (x1) -- node[right] {} (c2);
\draw[path,->] (x2) -- node[right] {} (c2);
\draw[path,->] (x3) -- node[right] {} (c2);

% c3
\draw[path,->] (x2) -- node[right] {} (c3);
\draw[path,->] (x3) -- node[right] {} (c3);
\draw[path,->] (x4) -- node[right] {} (c3);

\draw[path,->] (x1) -- node[right] {} (x1start);
\draw[path,->] (x3) -- node[right] {} (x3start);
\draw[path,->] (x4) -- node[right] {} (x4start);
\draw[path,->] (x4) -- node[right] {} (x4start2);

\end{tikzpicture}


==> overview_figures/two.tex <==
% fill white since these will be used in the foreground
\tikzset{box/.style={draw, thick, minimum height=1.8cm,minimum width=0.5cm}}
%\tikzset{main/.style={box,fill=gray!10}} %,label={below:{\text{Circuit} 1}}}}
%\tikzset{box/.style={font=\sffamily,draw, thick, minimum height=1.8cm,minimum width=0.5cm}}
%\tikzstyle{component}=[fill=white, font=\sffamily,draw, thick, minimum size=0cm,align=center]
\tikzstyle{component}=[fill=white, draw, thick, minimum size=0cm, align=center]
\tikzstyle{dest}=[fill=white, minimum size=0.5cm]

\begin{tikzpicture}[
	decoration={markings,mark=at position 0.6 with {\arrow{triangle 60}}},
	path/.style={thick},
	clip=false
	%path/.style={ultra thick,>=stealth,postaction=decorate}
	%every node/.style={
]

% BOXES IN THE BACKGROUND
\begin{pgfonlayer}{background}
\node[box, xshift=0cm, yshift=0cm, align=center, text width=2cm] (formula) {Formula $\phi$};
\end{pgfonlayer}{background}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% VARIABLES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\node[component,xshift=-3cm,yshift=-0.75cm]  (x1) at (formula.south) {$x_1$};
\node[component,xshift=1cm,yshift=-0.75cm]  (x2) at (formula.south) {$x_2$};
\node[xshift=-1cm,yshift=-0.75cm]  (bphantom) at (formula.south) {$\cdots$};
\node[component,xshift=3cm,yshift=-0.75cm]  (xn) at (formula.south) {$x_n$};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% START
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\node[dest,xshift=-1.5cm,yshift=0cm]  (start) at (x1) {start};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TARGET/FAIL FOR EACH VARIABLE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\node[dest,xshift=-0.5cm,yshift=-1cm]  (t1) at (x1.south) {target};
\node[dest,xshift=0.5cm,yshift=-1cm]  (f1) at (x1.south) {fail};
\node[dest,xshift=-0.5cm,yshift=-1cm]  (t2) at (x2.south) {target};
\node[dest,xshift=0.5cm,yshift=-1cm]  (f2) at (x2.south) {fail};
\node[dest,xshift=-0.5cm,yshift=-1cm]  (tn) at (xn.south) {target};
\node[dest,xshift=0.5cm,yshift=-1cm]  (fn) at (xn.south) {fail};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% EDGES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% phase 1
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% start to x1
\draw[path,dashed,->] (start) -- (x1);

% x_i to x_i+1
\draw[path,dashed,->] (x2) -- node[right] {} (xn);
\draw[path,dashed,->] (bphantom) -- node[right] {} (x2);
\draw[path,dashed,->] (x1) -- node[right] {} (bphantom);

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% phase 2
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% x_n back to formula
\draw[path,dotted,->] (xn.north) to[out=-270, in=45] (formula.north);

% formula to x_i
\draw[path,<-] (xn) -- node[right] {} (formula);
\draw[path,<-] (x2) -- node[right] {} (formula);
\draw[path,<-] (x1) -- node[right] {} (formula);
% edges to target and fail
\draw[path,->] (x1) -- (t1);
\draw[path,->] (x1) -- (f1);
\draw[path,->] (x2) -- (t2);
\draw[path,->] (x2) -- (f2);
\draw[path,->] (xn) -- (tn);
\draw[path,->] (xn) -- (fn);

\end{tikzpicture}

